Knowledge-Decks: Automatically Generating Presentation Slide Decks of Visual Analytics Knowledge Discovery Applications

Visual Analytics (VA) tools provide ways for users to harness insights and knowledge from datasets. Recalling and retelling user experiences while utilizing VA tools has attracted significant interest. Nevertheless, each user sessions are unique. Even when different users have the same intention when using a VA tool, they may follow different paths and uncover different insights. Current methods of manually processing such data to recall and retell users' knowledge discovery paths may also be time-consuming, especially when there is the need to present users' findings to third parties. This paper presents a novel system that collects user intentions, behavior, and insights during knowledge discovery sessions, automatically structure the data, and extracts narrations of knowledge discovery as PowerPoint slide decks. The system is powered by a Knowledge Graph designed based on a formal and reproducible modeling process. To evaluate our system, we have attached it to two existing VA tools where users were asked to perform pre-defined tasks. Several slide decks and other analysis metrics were extracted from the generated Knowledge Graph. Experts scrutinized and confirmed the usefulness of our automated process for using the slide decks to disclose knowledge discovery paths to others and to verify whether the VA tools themselves were effective.

==> paper/backup or references/1a_intro.tex <==

%%%%%%%%%%


% the  behavioral analyses do not yet fully use the previously listed knowledge models as a unified architecture to track and analyze users performing VA workflows. For instance, \citet{sacha2014knowledge} describes the conceptual relationship between \textit{Computer} and \textit{Human}, but how would one store the ongoing interactions within a graph structure~\cite{ansah2019graph}? Or, for what would one use this graph structure for behavior analysis?


% Although knowledge-related taxonomies, typologies, and ontologies are constantly referenced by VA research~\cite{sacha2014knowledge, federico2017role, sacha2018vis4ml, brehmer2013multi, polowinski2013viso}, the knowledge model as depicted in Fig.~\ref{fig:teaser}(A) is typically used as an underlying theoretical concept by researchers, leaving the work of putting it into practice to domain experts. Furthermore, there is a conceptual difference between the literature about \textit{workflow ontologies} and the literature on modeling VA as a knowledge model~\cite{chen2017pathways}. That is, the ontology research focuses on a taxonomy structure to describe the task sequence of VA workflows~\cite{sacha2018vis4ml, shu2006investigating} independent of the separation between \textit{Human} and \textit{Computer} processes, yet the knowledge models describe the iterative knowledge generation workflow between \textit{Human} and \textit{Computer}~\cite{federico2017role, sacha2014knowledge} without describing ways to perform behavior tracking or provenance analysis. 


% While the two have certain overlaps, these are mostly treated as limitations by their authors~\cite{xu2020survey, von2019informed}. Despite the significant impact and popularity of systems created using such works, the lack of a formal ontology that singlehandedly captures and compares a VA system's workflow to how and with what reason its users transform data into knowledge is a missed opportunity. Even works which pairs ontologies with \textit{Knowledge Graphs (KGs)} for analytical purposes~\cite{cashman2020cava, fujiwara2018concise, battle2019characterizing} can't analyse the VA workflow in its entirety. In other words, even though we have access to literature with well-built models and applications, no methodology provides a way to simultaneously understand on a per-user basis how past knowledge aided in generating new knowledge, to identify the workflow which lead to such knowledge, to compare multiple user's intentions and behavior patterns, to relate them to a VA workflow's \textit{state space}, to generate the full user and computer interactivity patterns during the workflow and which allows its further customization and analysis.

% In light of this, we propose \textit{Visual Analytic Knowledge Graph (VAKG)}, a multi-layer ontology architecture based on \textit{Temporal Knowledge Graphs (TKG)}~\cite{gottschalk2018eventkg}. \textit{VAKG proposes to structure the knowledge gathering process within the Visual Analytics (VA) life-cycle into a set of linked knowledge graphs}. For this, VAKG describes a model which systematically stores, describes, and enables analysis of the tasks done by a user and their generated knowledge during any given VA workflow (Fig.~\ref{fig:teaser}). As our core contribution, VAKG introduces the concept of a \textit{multi-lane TKG model} (Fig.~\ref{fig:teaser}(B)), which unfolds the VA typology states over time while keeping the separation between \textit{Human} and \textit{Computer} concepts and between the \textit{sequential} and the \textit{state space} aspects of a VA workflow, resulting in a knowledge graph (Fig.~\ref{fig:teaser}(C)) which provides an architecture for VA systems to structure, store and link users' knowledge generation workflows, all computer-side changes over time and the relationship between users' reasoning and the executed workflow. Additionally, VAKG's multi-layer approach allows all parties to attach existing models to VAKG as sub-components, including graph analysis techniques. 
% % TODO: eu juntei aqui denovo.. melhor fazer o q?
% Although VAKG seems to compete with current knowledge models and knowledge graphs within VA, our purpose is not to replace existing models but to describe an architecture where such models can overlap and communicate through our multi-layered knowledge graph architecture since it allows for a flexible definition of sub-ontologies to be used within VAKG.

% The remainder of the paper is structured as follows. In Sec.~\ref{sec:related}, we discuss related work involving techniques that seek to formalize the VA knowledge flow as a concrete framework, usages of knowledge graphs within VA, including how they differ from VAKG, and other concepts which tackle the ongoing knowledge evolution during data analysis. In Sec.~\ref{sec:methodology}, we extend the existing works of the theoretical knowledge model of VA to formalize VAKG. In Sec.~\ref{sec:comparison}, we present possible applications of VAKG while comparing with existing methods and justifications for further extending VAKG. We also illustrate the potential impact of using VAKG by interviewing two experts: one in the food-business field who routinely performs manual financial data analysis for decision making and another who manages a fraud detection and credit analysis area within a large bank in Sec.~\ref{sec:interview}. Finally, in Sec.~\ref{sec:future} we discuss VAKG current limitations and the next steps within our research plan and in Sec.~\ref{sec:conclusion} we draw our conclusions.

%%%%%%%%%%%%%%

Visual Analytics (VA) systems provide ways for users to harness insights and knowledge from datasets~\cite{sacha2014knowledge}. 

The understanding of what knowledge is, how it is formed, and how one can model such knowledge generation into a shareable format has been much investigated within VA~\cite{collins2018guidance}, Knowledge Graphs (KGs)~\cite{chen2020review, xu2020survey}, Semantic Web~\cite{ferrara2011data} among other fields. Seen that VA is understood as the means for users to generate and amass knowledge through visual interactivity~\cite{collins2018guidance}, VA researchers have been using existing knowledge models~\cite{sacha2014knowledge, federico2017role} and ontologies~\cite{sacha2018vis4ml} as a guide for developing knowledge-centric VA. For instance, the literature describe VA as an iterative process between users and computers~\cite{federico2017role}, as a taxonomy of knowledge~\cite{chen2017pathways, andrienko2018viewing, von2014interaction}, or as an ontological structure~\cite{sacha2018vis4ml, chen2017pathways}. In parallel, VA has also shown that insights about a VA tool or its users can be found by tracking and analysing users' behavior, interactivity and insights using \textit{provenance} analysis~\cite{heer2008graphical, battle2019characterizing}. However, these behavioral analyses do not yet fully use the previously listed knowledge models as a unified architecture to track and analyze users performing VA workflows. For instance, \citet{sacha2014knowledge} describes the conceptual relationship between \textit{Computer} and \textit{Human}, but how would one store the ongoing interactions within a graph structure~\cite{ansah2019graph}? Or, for what would one use this graph structure for behavior analysis?

For instance, \cite{collins2018guidance} describe in detail what intelligent guidance is and how it provides digestible and interpretable information to users from visualizations and from results of machine learning techniques. For instance, a tool applies intelligent guidance by reducing the cognitive load and visual bias that users interacting with a visual analytic tool may experience. Since the analysis of users' behavior is dependent on their pre-conceived tacit knowledge~\cite{federico2017role} and their own interest when starting an analysis process, \cite{collins2018guidance} also describe a user knowledge model where VA is the means for users to generate and amass knowledge through visual interactivity. In this context, the authors describe KGs as an abstract representation of user-generated knowledge. 



%%%%

Despite the significant impact and popularity of systems created using such a conceptual model, the lack of a formal methodology to capture how users transform data into knowledge is a missed opportunity. Researchers do not currently have access to any existing method of knowledge modeling to attach their tool as an external dependency. Most of the existing tools do not record users' interactions, with even fewer recording the constant influx of new insights from the user, and rarely linking the two. In this way, most systems are not capable of recording and analyzing the user's transitions between insights into knowledge, nor have strategies to help to understand how well past knowledge aided the user in generating new knowledge, nor how to compare multiple user's usage patterns, nor how to leverage previous user's insights and usage patterns to enhance a new user's experience. %Moreover, there is seldom any attempt to implement this knowledge modeling theory into a temporal framework. 

Nevertheless, there are many valuable applications for a method that can represent and record the user's knowledge generation process. For instance, most VA systems or applications within the literature are expected to have user evaluation. However, the usual procedure is for the researcher to collect user evaluation data, such as user interactions while using the system, and after applying statistical analysis, the researcher has the results. Since the researcher already has to collect both the system's usage and user feedback, why is this step not built into every VA tool by default? Another relevant example is Exploratory Data analysis tasks (EDA), where users' interactivity generates insights~\cite{keim2010visual}, but this process is rarely tracked and analyzed through a formal method. Many other examples can benefit from it, such as cooperative analysis through CSCW~\cite{shi2019visual}, where the interactivity of one use may aid others through recommender systems, and active learning methodologies~\cite{legg2019visual}, where users directly provide new knowledge to the system. Although the knowledge generation process from Sacha et al.~\cite{sacha2014knowledge} is the backbone of current VA tools, these tools have yet to fully utilize the knowledge model structure as a means to gather and analyze user data.

In light of this, we propose \textit{Visual Analytic Knowledge Graph (VAKG)}, a temporal knowledge model framework based on \textit{Temporal Knowledge Graphs (TKG)} and the aforementioned knowledge modeling methods~\cite{federico2017role}. VAKG systematically stores, describes and enables analysis of the knowledge generated by users during any given VA task (Fig.~\ref{fig:teaser}). VAKG introduces the concept of a \textit{TKG modeling} (Fig.~\ref{fig:teaser}(B)), which unfolds the human and computer states over time and models the unfolded graph into the knowledge graph architecture (Fig.~\ref{fig:teaser}(C)) in order to provide a systematic framework for VA tools to structure their user's knowledge generation workflow, store their user's ongoing knowledge gain and provide means for all parties to analyze and use the TKG. 

VAKG is designed as a framework that collects and analyzes a given tool's usage data and user knowledge evolution. VAKG bridges the gap in the current understanding of knowledge during VA development, the theoretical VA knowledge framework of Federico et al.~\cite{federico2017role} and Sacha et al.~\cite{sacha2014knowledge}, the analysis of user's knowledge gain over time, and the methodology of knowledge structuring, storage, and analysis processes of Knowledge Graphs. We also propose a sample system called VAKGI, which minimally implements this framework as a general-purpose web service. 

The remainder of the paper is structured as follows. In Sec.~\ref{sec:related}, we discuss related work involving techniques that seek to formalize the VA knowledge flow as a concrete framework, usages of knowledge graphs within VA, including how they differ from VAKG, and other concepts which tackle the ongoing knowledge evolution during data analysis. In Sec.~\ref{sec:methodology}, we extend the existing works of the theoretical knowledge model of VA in order to formalize VAKG and VAKG extensions mathematically. In Sec.~\ref{sec:extensions}, we present possible applications VAKG, justifications of further extending VAKG, a sample implementation of VAKG called VAKGI as a web-based system, and the practical comparison between the regular data analysis done by an expert in the food-business field who routinely performs manual financial data analysis for decision making and the VAKG framework. Finally, in Sec.~\ref{sec:future} we discuss VAKG current limitations, potential usages, and the next steps within our research plan, and finally, in Sec.~\ref{sec:conclusion} we draw our conclusions.

==> paper/backup or references/3_related.tex <==
\section{Methodology}\label{sec:methodology}

To arrive at VAKG's goals and ontology, we first formalize and describe the Visual Analytics (VA) knowledge model framework~\cite{sacha2014knowledge, federico2017role} and its role in VA ontologies~\cite{xu2020survey, sacha2018vis4ml}. Then, following the example of related works, we use this foothold to unfold the Human-Computer loop into a temporal sequence of states, as is shown in Fig.~\ref{fig:teaser}(B). We then discuss VAKG goals in light of related work limitations, and, to achieve these goals, we expand the ontology and use a \textit{Temporal Knowledge Graph (TKG)} structure to allow VAKG to store and analyze the user's knowledge gain process.

\subsection{Background and Goals}\label{sec:formal}

The theoretical background of VA's knowledge model is a foundation work for most, if not all, research within VA. The rather simplistic representation of this model shown in Fig.~\ref{fig:teaser}(A) characterizes its two main actors: \textit{Humans} and \textit{Computers}. From \citet{sacha2014knowledge}, VA's cyclical process of human-computer interactions and feedback loops describes that knowledge is generated over time. \citet{federico2017role} expand these concepts by describing the inner taxonomies of both Human and Computer sides and further describing that depending on the system and use-case, different styles of interaction loops can be described through these inner taxonomies. They also propose a mathematical interpretation called ``Conceptual Model of Knowledge-Assisted VA'' to describe a base knowledge model, which is then used t construct many derived models, such as knowledge generation, conversion, internalization, externalization, and exploitation. For our purposes, the essential information extracted from these works is that VA workflows have many well-defined inner taxonomies, which may vary depending on the application and use case. Still, there always exists an overarching human-computer interactivity loop.

As discussed previously, such theoretical models are also applied in practice either by using the theory as an inspiration for design guidelines or through formal ontologies. For instance, \citet{sacha2018vis4ml} describes an ontology of the knowledge model as what they call a ``diamond feedback loop'', and \citet{battle2019characterizing} uses the knowledge model as an inspiration to record user behavior as a graph network for analysis. In all cases, the interactivity loop between \textit{Human} and \textit{Computer} is always present. 

To better understand VAKG's goals, we extract the underlying ontology of the knowledge model from these existing works following the Web Ontology Language (OWL)~\cite{chen2017pathways}. By pairing the temporal aspect of the human-computer interactivity loop from knowledge models~\cite{sacha2014knowledge, federico2017role} and the ``diamond rule'' of \citet{sacha2018vis4ml}, we define the sequences of \textit{State} classes (green circles) with two main sub-types: \textit{Human States} (red outline) and \textit{Computer States} (black outline), as is seen in Fig.~\ref{fig:teaser}(B). 

Next, we incorporate the temporal aspect into the ontology. For this, we follow the current conceptual work of defining and characterizing VA workflows (see ~\ref{sec:related}). Although many specific ontologies of relationships have been designed recently, we first return to the roots of VA and focus our macro design on the temporal relationship between the two aforementioned classes as the design core of VAKG. Formally speaking, we define two relationships that connect the aforementioned two \textit{state} types: \textit{interact-Human-Computer} and \textit{feedback-Computer-Human}, similar to~\cite{sacha2018vis4ml, shu2006investigating}, as is seen by the red-dashed and black-dashed lines of Fig.~\ref{fig:teaser}(B). These relationships are analogous to \textit{has-IO-Entity-Successor}, and \textit{has-Process-Successor} of \citet{sacha2018vis4ml} and, just as they argue, this allows for ``directed connections explicitly define the predecessor-successor and action-actor relationships within any workflow''. Therefore, by just extracting the descriptors from existing works~\cite{sacha2018vis4ml, federico2017role}, VAKG ontology should include:

\squishlist

\item \textbf{\textit{Human} Class (H):} All human-related information and changes, such as tacit knowledge, newly gained insights and findings, perception/cognition of the user, user's will or wishes while performing any task, any questions or goals the user may have and all demographic information on the user.

\item \textbf{\textit{Computer} Class (C):} All computer-related information and changes, such as datasets, metadata, visual and interface state at a given time, machine learning state, automated processes, system specifications, system configuration, and available explicit knowledge.

\item \textbf{Relationship \textit{interact-Human-Computer}:} \textit{What} and \textit{how} has the user interacted or changed within the interface (Computer) and \textit{why} has the user interacted with the interface (Computer) at a given time.

\item \textbf{Relationship \textit{feedback-Computer-Human}:} \textit{How} was the state of the Human prior to the changes in the interface at a given time.

\squishend

%FVP.: você tirou essa lista de algum lugar ou se baseou em algum lugar para defini-lá? Se sim, seria bom dar as referências.

So far, we have defined what already exists in the literature~\cite{sacha2018vis4ml, federico2017role}. However, as we have discussed in Sec.~\ref{sec:related}, the related works have an ambiguous definition of the two classes and two relationships: whether the \textit{knowledge gathering} process is to be considered temporal or not. A temporal process is a provenance workflow that considers the sequences of interact-feedback loops as sequences of events over time, which can then be modeled through taxonomies~\cite{sacha2014knowledge, federico2017role, polowinski2013viso, von2014interaction} or systematically used for tracking or analysis~\cite{battle2019characterizing, xu2020survey, fujiwara2018concise, bernard2017comparing}. On the other hand, an atemporal process would instead consider the \textit{state space} of the VA workflow. 

We consider a \textit{state space} a set of some or all possible configurations of a system or entity and all the immediate adjacency relationships between such configurations. For example, a state space can be a graph network with a node for every possible state a VA tool can be and a link between every two nodes that are a single event or interaction away from each other. Interpreting the ontology described above as a state-space has been considered in some examples of theoretical works~\cite{sacha2018vis4ml, von2019informed} and analysis-focused works~\cite{battle2019characterizing, clifton2012advanced}. However, even when both temporal and atemporal aspects are used, it is ambiguous or uncertain how the two are differentiated and whether they are connected in any way, as we have discussed in Sec.~\ref{sec:related}. Furthermore, the inner elements of the Human side versus the Computer side of VA are not always separated within these works, which creates further ambiguity. For instance, while theoretical works~\cite{sacha2014knowledge, federico2017role} clearly separate the two in their models, works describing VA ontologies~\cite{sacha2018vis4ml, brehmer2013multi}, user-tracking~\cite{bernard2017comparing} and behavior analysis~\cite{battle2019characterizing, xu2020survey} usually merge the two sides or ignore one side completely.

With this, we have our core goal stated: \textit{VAKG is an architectural framework designed with ontologies that formally models the temporal sequences and the state space of both the Computer and Human sides of a VA workflow, and when used to record VA workflow sessions, it directly allows for provenance and state space analysis}. Note that VAKG should be understood as an ontology \textit{architecture}, in the sense that it is not a static ontology but is expected to be expanded and specialized for different use-cases. With that in mind, our objectives while designing VAKG are to:

\begin{itemize}
    \setlength\itemsep{0em}
    \item[\textbf{G1:}] Create an ontology that describes and links all four VA workflow aspects:
    \begin{itemize}
        % \setlength\itemindent{-1em}
        % \setlength\leftmargin{-1em}
	    \item[\textbf{G1.1:}] Temporal sequences of knowledge gathering per user (Human State Provenance).
        \item[\textbf{G1.2:}] The user feedback and insights which occurs within a VA workflow (Human State Space).
        \item[\textbf{G1.3:}] The Computer state space within a VA workflow (Computer State Space).
        \item[\textbf{G1.4:}] Temporal sequences of computer events/tasks which are executed during VA workflow sessions (Computer State Provenance).
    \end{itemize}
    \item[\textbf{G2:}] Architect such ontology so that it can be used to record users executing a VA workflow and allow its analysis.
    \item[\textbf{G3:}] Have the ontology able to optionally incorporate lower-level ontologies and models for specific analytical use-cases.
\end{itemize}

\subsection{VAKG Expanded Ontology}\label{sec:vakgkg}
\subsubsection{Temporal Disambiguation}

So far, we have extracted an ontology from the literature~\cite{federico2017role, sacha2018vis4ml} and discussed its ambiguities regarding whether the \textit{knowledge gathering} process is temporal (e.g., provenance) or not (e.g., state space). To solve them, VAKG expands the ontology described above by explicitly separating the concepts of temporal and atemporal relationships. This is done by interpreting the two relationships, namely \textit{feedback-Computer-Human} (\textbf{G1.2}) and \textit{interact-Human-Computer} (\textbf{G1.3}), as atemporal relationships and adding two more relationships for temporal connections:

\squishlist

\item \textbf{Relationship \textit{update-Computer-Computer}:} Time-stamped indication of \textit{What} changed in the interface and \textit{why} did this change happen (\textbf{G1.1}).

\item \textbf{Relationship \textit{insight-Human-Human}:} Time-stamped indication of \textit{what, how and why} has the user aggregated as new insights/findings from the new information (\textbf{G1.4}).

\squishend

Our expanded version of the VA workflow ontology shown in Fig.~\ref{fig:teaser}(B) attempts to reduce, if not eliminate, this ambiguity. The figure shows the two temporal relationships as the light-red and gray diamond arrows. In contrast, the atemporal relationships are the red and black dotted arrows. A parallel mathematical formalization of the same ontology is discussed in the supplementary material.

\subsubsection{The Update Sequence}\label{sec:updateseq}

Therefore, although the basic architecture of VAKG follows existing research, it also attempts to solve existing temporal versus atemporal issues. Even though analysis of the temporal aspect of VA, such as knowledge gathering or data provenance, is at the center of VAKG's goals, the ontology so far does not fully depict a timeline of events separate from a timeless ontology of possible events (\textbf{G1}). For this and for VAKG to also allow for analytical tasks to be done (\textbf{G2}), we propose that the design of VAKG follows existing research on \textit{Knowledge Graph (KG)} . 

A KG is a graph structure where knowledge reasoning is modeled as connections between classes or properties, such as ``George Washington \textit{is a} human'' and ``Canada \textit{is a} country''. A \textit{Temporal Knowledge Graph (TKG)}, however, models these connections as the temporal relationship between the classes or properties. Many different types of TKGs exist. For each, this temporal connection has a different meaning. For instance, the most used version of TKGs uses time as the connection, where two connected nodes represent two events that co-occurred. An example of such a KG would be all purchases done between different businesses within a supply chain, where the product ``Mayonese'' may have been bought by a store ``Wallmart'' from the seller ``Hellmann's'' on ``25/06''. In this TKG, the connection between the three nodes: Wallmart, Hellmann's, and Mayonnaise, would be ``25/06''. To design such structures, one must use Web Ontology Language (OWL) or a similar ontology language~\cite{chen2017pathways}. By designing VAKG's ontology with KGs and TKGs in mind, we enable easier ways for both temporal and atemporal visualization and analysis to be done with VAKG through existing works~\cite{chen2020review, wang2018ripplenet, han2014chronos, gottschalk2018eventkg, cashman2020cava}.

VAKG is arguably more complex than the KG examples given so far. When also considering the four different aspects listed within \textbf{G1}, we describe VAKG as a 4-lane KG, with one lane for each of the four aspects of \textbf{G1}. However, our ontology of Fig.~\ref{fig:teaser}(B) does not match this expectation. For that, we create a new ontology by enhancing the two temporal relationships into its own \textit{class} which represents an \textit{Update} process (Fig.~\ref{fig:teaser}(C)). We, therefore, modify the relationship between two \textit{States} of the same type (e.g., \textit{Human-Human}) to become a new \textit{class} of type \textit{Update} and, from this, three new relationships are created: \textit{does-State-Update}, \textit{leads-Update-State}, and \textit{follows-Update-Update}, which forms the 4-lane TKG architecture of Fig.~\ref{fig:teaser}(C). With this, the \textit{Human Update} inherits the definition from \textit{insight-Human-Human}, and the \textit{Computer Update} inherits the one from \textit{update-Computer-Computer}. A representation of how the \textit{classes} relate to each other can be seen in Fig.~\ref{fig:entiredesign}, where it is shown that there are four \textit{classes}: \textit{Human State}, \textit{Human Update}, \textit{Computer State}, and \textit{Computer Update}. This now achieves \textbf{G1}, since the \textit{Human Updates TKG} identifies \textit{Human State Provenance}, the \textit{Human States KG} identifies the \textit{Human Space State}, the \textit{Computer State KG} identifies the \textit{Computer State Space} and the \textit{Computer Update TKG} identifies \textit{Computer State Provenance}, all of which describe \textit{one overarching TKG with 4 sub-KG lanes}. VAKG representation of Fig.~\ref{fig:teaser}(C) simplifies this definition as: \textit{Feedback} lane for Human States, \textit{Interactivity} lane for Computer States, \textit{Update Interface} lane for Computer Updates and \textit{Knowledge} lane of Human Updates. 
%: a TKG for \textit{Human State Provenance}, one KG for \textit{Human State Space}, one KG for \textit{Computer State Space}, and one TKG for \textit{Computer State Provenance}}. 

\begin{figure}%[tb]
    \centering
    \includegraphics[width=.75\columnwidth]{pictures/fullVAKGontology.PNG}
    \caption{VAKG ontological design. The four different lanes of VAKG are represented. Two are KGs that describe the possible states of the inner property-maps or sub-graphs. Two are TKGs describing the sequences of updates, such as the sequence of insights and knowledge-gain by users in a VA workflow or the sequence of computer events. }
    \label{fig:entiredesign}
\end{figure} 

% \begin{figure}%[tb]
%     \centering
%     \includegraphics[width=.9\columnwidth]{pictures/vakgsimple.PNG}
%     \caption{Simple VAKG examples. In (A), a user performed 3 operations in the VA tool ($U_{\{1,2,3\}}^{va}$), changing the state of the VA tool $C_t^{va}$. In parallel, the user started with previous tacit knowledge $C^u_1$ and through a sequence of findings and insights $U^u_t$, they reached the end of the analysis at $C^u_4$. Similarly, in (B) two different users performed the exact same interactions through the same sequence of findings and insights as each other. }
%     \label{fig:vakgsimple}
%     \vspace{-0.65cm}
% \end{figure} REINCLUDE SOMEWHERE? does not fit..

\subsubsection{VAKG Property Map and Data Collection}\label{sec:propertymap}

So far, we have focused on the VAKG structure. Still, an integral part of our proposal is to record users executing a VA workflow and allow its usage for analysis (\textbf{G2}). While the usual way of thinking on ontology design is to focus on OWL classes and their relationships, with VAKG we are also utilizing OWL \textit{class properties}, sometimes called \textit{data properties} or, when used within the context of KGs, \textit{property-maps}. This design pattern uses the idea that every class in OWL can contain inner properties with attached data. The \textit{property-map} design patterns is, however, interchangeable with the design pattern of pure OWL classes and relationships~\cite{myroshnichenko2009mapping}, which removes any potential limitation on interconnecting our design with other ontologies.

As per our design, each node within VAKG holds a property map of all the node information. Fig.~\ref{fig:vakgexpatt} shows a simple example of what this property map is when using VAKG to model an \textit{Exploratory Data Analysis (EDA)} task. 
%which is a type of VA workflow that allows users to gain knowledge by interactively explore data without pre-determined guidance~\cite{st1998intelligent, keim2010visual}. 
%
%FVP.: acho que nao precisa, quem vai ler tem que saber o que é EDA.
%
However, how much of the recorded information should be stored in the property map? Although theoretically, one could store all information related to a given state down to the exact bits within the Computer State or a brain scan of a Human State, we understand that it is not reasonable to expect that every VA workflow requires such an amount of information. Therefore, we define as part of VAKG that the property map of a State should, at the very least, uniquely identify that specific State within the state space of VAKG.

Through this definition, we can see that a given Computer or Human \textit{States} can repeat if the same conditions occur multiple times. For instance, if the user within an EDA task performs a sequence of interactions that returns all the visualizations to an already explored state, the VAKG's \textit{Computer States} would describe the state transitions that the user took until he returned to that state. Though less common, this property is shared by the \textit{Human States}, where the user could have had an insight previously, and after further EDA interactions, s/he simply had the same insight once again. This, however, is not a property shared by the Computer or Human \textit{Update} sequences. By applying the same definition to the two \textit{Update} classes, their expected property-map would uniquely identify the changes between the two Computer or two Human \textit{States}, which, for VAKG, would include the timestamp of when the change occurred. 

Therefore, it is important to note that the Feedback and Interactivity lanes pf Fig.~\ref{fig:teaser}(C) are not \textit{temporal} because their connection is not temporally dependent but only dependent on the adjacency of their inner property-maps. Nevertheless, we still describe VAKG as a TKG as a whole due to the other two lanes, which are themselves a \textit{temporal} sequence of events. With this, the example of an EDA task shown in Fig.~\ref{fig:vakgexpatt} can be better understood through this 4-lane interpretation of VAKG.

\begin{figure}%[tb]
    \centering
    \includegraphics[width=\columnwidth]{pictures/VAKG_abstract.png}
    \caption{A VA tool called ExPatt used VAKG to track its interface states and user's knowledge gain. The tool's state is stored as a property map, and on each update operation (e.g., an interaction on the tool) a new update node records all pertained information. Similarly the user's ongoing insights and tacit knowledge follows in a separate timeline.}
    \label{fig:vakgexpatt}
\end{figure}


VAKG itself does not strictly design the property-map typology because each use case will have different requirements (\textbf{G3}). For instance, Vis4ml~\cite{sacha2018vis4ml} focuses on designing an ontology which describes the workflow of VA-assisted ML. As we discussed before, although Vis4ml achieves very well its own goals, its ambiguity of temporal and atemporal aspects limits its usage when compared to VAKG. However, our design also expects that Vis4ml may use their work to extend VAKG's ontology through, for instance, defining the content of all property-maps within each \textit{State}. As an example, Vis4ml could specify a property-map which describes the exact state of ``Prepare-Data'' at a given time, including all statistical profiles, data processing, and annotation. Another possibility is to instead of defining property-maps, they could upgrade the \textit{Computer States} into their own Vis4ml ontology (\textbf{G3}). 

Using an existing ontology or taxonomy map, such as Vis4ml, as a relationship model of the property-map within a \textit{Class} is interesting in some use cases. For instance, by following the previous example, we know that Vis4ml~\cite{sacha2018vis4ml} has a relationship model within all ``Prepare-Data'' nodes. Therefore, if a single \textit{Computer state} can define the state space of an entire ``Prepare-Data'' process, the user of VAKG can choose to expand the property-map into a sub-KG containing a full ontology within. This same concept can be applied to Human or Update \textit{States}, where complex knowledge models from \citet{federico2017role} can be used. Further examples and applications will be discussed in Sec.~\ref{sec:comparison}.

% \begin{figure}%[tb]
%     \centering
%     \includegraphics[width=\columnwidth]{pictures/tempsubkg.png}
%     \caption{A given state can either have a property-map or be connected to a sub-KG which contains an ontology of its own (num cabe...}
%     \label{fig:subkg} num cabe
% \end{figure}

\subsubsection{Temporal Misalignment}\label{sec:summarization}

The examples of VAKG given so far through Fig.~\ref{fig:teaser} show a new Human update for every new Computer update. In other words, these examples expect users to have a new insight/finding at every single interaction, forcing these Update states to align perfectly. This, however, does not reflect the current literature, as is shown in manual and automatic annotations research~\cite{yu2019flowsense, kim2020answering, mogadala2019trends, mathisen2019insideinsights}. In reality, users may have one intention or insight that causes multiple interactions within the VA tool. After all these interactions, the user finally generates a new piece of knowledge. Users may also have multiple insights or intentions after performing a single interaction. With this in mind, VAKG does not require exact parity between the Computer and the Human timeline. In place of this, VAKG interprets the Update states as the summary of all changes between the two states. These Updates may be linked to one or more Updates from the parallel Update lane. For instance, Fig.~\ref{fig:vakgsummary} exemplifies when two users perform multiple actions only to harness a single piece of new information at the end. A single insight Update is linked to three interface Updates in this example.

\begin{figure}[tb]
    \centering
    \includegraphics[width=.68\columnwidth]{pictures/vakgsummary.png}
    \caption{VAKG summary extension. Although the two users performed three actions (black border), the two users had only one intention from the beginning and learned something new only at the very end (red border). Relationships between the Computer lane (left) and Human lane (right) occur between nodes of the same inner color.}
    \label{fig:vakgsummary}
    % \vspace{-0.65cm}
\end{figure}

This loosens the definition of the relationships between the Update classes. More specifically, we extend the definition of the \textit{knowledge lane} to be related to any number of updates in the tool. Similarly, a single interaction can also be related to any number of new insights of the \textit{knowledge lane}. This forces VAKG to handle new updates separately between the Computer and Human classes. Still, the resulting KG may be closer to how exactly the users' knowledge gain happened. We define this aspect of VAKG as the \textit{summarization} or \textit{interpolation} of Update nodes. Arguably, this also reduces the amount of information within VAKG since when multiple interactivity Update classes link to a single knowledge Update class, the ontology will not retain how each of the interactions uniquely impacted the property-map of the knowledge Update. Although this limits certain aspects of VAKG, as we have discussed before, specific use-cases can upgrade the property-map of a \textit{summary Update} into an inner ontology which enables further information to be modeled within the TKG.

==> paper/backup or references/3b_related.tex <==
\section{Background and Related Work}\label{sec:related}

For the design of our system, we have used a modeling process based on existing knowledge model research, with which we implemented ways to collect user data and transform it into a retelling of the users' insights and knowledge discovery process. Therefore, this section will discuss VA knowledge models and their practical usage when applied to knowledge discovery. Then, we discuss several provenance~\footer{Provenance: tracking and using data collected from a tool's usage~\cite{ragan2015characterizing}} approaches, including data and analysis provenance which allows us to collect users' insights and knowledge discovery process. Finally, we discuss existing approaches to recall and retell users' knowledge discovery as storytelling presentations.
% TODOLC: explicar o q eh provanence rapidao| fiz na intro
% TODOLC: muda a estrutura pra ser 2: modeling adn provenance VS knowledge discovery recall and explanation
% \fvp{e artigos sobre o nosso objetivo? tem que falar alguma coisa aqui.}

\subsection{Knowledge Modeling and Provenance in VA}
\fvp{modelagem do usuario (lc: e da ferramenta tambem) - VAKG}

VA literature in knowledge modeling has shown that users' interactivity with VA tools can be modeled as an iterative workflow of user intentions, behaviors, and insights~\cite{sacha2014knowledge, sacha2016analytic, federico2017role}. For instance, Federico et al. ~\cite{federico2017role} describes how VA tools and frameworks can be modeled following said knowledge modeling methodology. They also describe how to interpret VA research in light of their model. This methodology of describing VA as an iterative workflow of events between Human and Machine actors shows that it is possible to understand a VA problem as a sequence of events. Additionally, this model can also represent automatic processes, such as data mining or machine learning, as part of the sequence of events, even if it was not triggered by a Human interaction. Sacha et.al.~\cite{sacha2018vis4ml}, among others, show through their detailed machine-learning ontology that these Computer-generated events permeate much of VA as a whole. 

% Nevertheless, although these works demonstrate how their model matches VA, they do not discuss how to take advantage of these models to design a new system or tool, nor to what advantage one would do that. As far as the authors are aware, there exists little discussion of how to use these theoretical knowledge models and ontologies to give an advantage to a newly built tool. % REMOVE because it is useless for this work
%
% \fvp{porque vc critica isso? nao eh esse seu objetivo. Aqui acho que nao precisa criticar nada, soh dizer o que usamos disso tudo, ou como isso se encaixa na nossa ideia eh o suficiente. De fato isso nao sao RW mas background. }
% TODOLC: podemos fazer um paragrafo falando como usaremos isso antes de criticar
%
% \subsection{Provenance and User Tracking in VA}

\fvp{identifcar e extrair info - anotacao}


Usually, VA developers and researchers use more practical means to model, collect, store, and utilize their tools or users' experiences. For instance, some researchers collect and analyze user behavior using provenance~\cite{da2009towards, ragan2015characterizing}. For example, Landesberger et.al.~\cite{von2014interaction} perform behavior provenance by modeling user behavior as a graph network, which is then used for analysis. Other works also use graph networks as a way to model knowledge~\cite{fensel2020introduction}, data provenance~\cite{simmhan2005survey, da2009towards}, insight provenance~\cite{gomez2014insight}, and analytic provenance~\cite{xu2015analytic, madanagopal2019analytic}. All these tools and techniques aim to collect some part of the user's knowledge discovery process and model it into some structure.

Among these, graph networks, or more specifically knowledge graphs~\cite{fensel2020introduction, guan2022event}, are uniquely positioned as a means to model the user's knowledge discovery process due to their specific applicability in collecting and analyzing two kinds of data: temporally-based event data~\cite{guan2022event} and relationship-centric data~\cite{auer2007dbpedia}. Since VA is modeled based on events~\cite{sacha2014knowledge, federico2017role} and our goal is to find and analyze the \textit{relationship} between VA events~\cite{fujiwara2018concise}, we decided to use knowledge graphs as one of the cornerstones of our system.

In order to perform provenance, however, one must first collect information from the user. Existing works have collected changes in datasets~\cite{da2009towards}, updates in visualizations~\cite{battle2019characterizing, xu2020survey}, and other similar events in order to recreate and recall user behavior. On the other hand, tracking user's \textit{Tacit Knowledge} as defined by Federico et al. ~\cite{federico2017role} is either done by manual feedback systems~\cite{bernard2017comparing, mathisen2019insideinsights}, by manual annotations over visualizations~\cite{soares2019vista} or by inference methods that attempt to extract users' insights by recording the users' screens, video or logs and extract from them interactivity patterns as a post-mortem task~\cite{battle2019characterizing, guo2015case}. Among these VA systems, InsideInsights~\cite{bernard2017comparing} is an approach to recording insights through annotations during the user's analytical process. They have demonstrated that collecting user annotations is a legitimate way to extract and store user insights.

% \fvp{de novo, a gente critica algo que a gente nao quer resolver. A nossa critica deveria ser em como o que eles fazem se conecta com a transmissoa de informacao. Ou entao, dizer como a gente usa isso como parte da nossa solucao.}
% TODOLC: podemos fazer um paragrafo falando como usaremos isso antes de criticar

% \subsection{Knowledge Graph for Modeling Users' Knowledge Discovery Process}

\fvp{armazenamendo da informcao de anotacao e interacao do usuario - provenance}



After collecting data from users' knowledge discovery process, one must impose a structure to it. For that, the design of knowledge ontologies has been a central goal of \textit{Knowledge Graphs} (KGs)~\cite{fensel2020introduction}. KGs~\cite{chen2020review, guan2022event} is a widely used technique to store knowledge in a structured format and has shown many successful methods of how to interpret, store and query explicit knowledge, such as the information within Wikipedia~\cite{auer2007dbpedia}. KG methodology defines that the relationships between nodes of a graph network, and not just the nodes themselves, can represent knowledge~\cite{guan2022event}. Among similar structures, Event Knowledge Graphs~\cite{guan2022event} expands on this concept by including the concept of event-based data, defining that paths of the graph's relationships represent sequences of events over time.

In order to store and analyze a KG, graph databases, such as neo4j~\cite{noauthororeditorneo4j}, have emerged with a wide array of available techniques. Such specialized databases are needed since the structure of KGs focuses less on the usual transactional or row-based structure of typical relational databases and their transactional structure~\cite{cashman2020cava}. Applications of KGs are also part of the overall graph network research, which means that graph network techniques such as Graph Neural Networks (GNNs)~\cite{jin2020gnnvis}, graph visualizations~\cite{chang2016appgrouper, he2019aloha} and graph operations~\cite{ilievski2020kgtk}, such as page rank and traveling salesman, can be applied to KGs.

Among works that utilize KGs to model and store the user's knowledge discovery process, we must highlight VAKG~\cite{christino2022data}. This conceptual framework connects the VA knowledge modeling theory with KGs to structure and store knowledge provenance. Indeed, as later discussed, our solution is built around the VAKG methodology. We have modeled two existing VA tools in light of existing knowledge models. From it, we have developed a KG ontology (or schema) to store users' knowledge discovery process. With VAKG we can identify what should be collected from the user. However, it by itself does not aid in performing data collection, nor aids in defining how to analyze and extract slide decks from the generated KG.
%
\fvp{nao sei se vale a pena falar de slide deck, mas talvez de como divulgar o conhecimento acumulado no grafo.}


Certain limitations from these works show that tracking automatically-generated insights~\cite{spinner2019explainer} or accounting for automatic computer processes~\cite{federico2017role} is still a challenging and largely unsolved problem. Therefore, we have opted in our system to follow the argumentation of Xu Et.Al.~\cite{xu2015analytic} and focused on manual means to collect user insights and intentions while providing automatic collection of computer-processes~\cite{federico2017role} and automatic linking of all user-related to its respective computer-related events~\cite{christino2022data}. %We argue that this challenge is due to these tools not being developed based on the VA knowledge model. Instead, they only focus on collecting an incomplete view of the knowledge discovery process, showing the need for more integration between existing VA tools, provenance techniques, and modeling methodologies discussed.

% \subsection{Recall of the Knowledge Discovery Process}
% LC: pessoalmenet axo melhor nao colocar uma secao aqui, mas o q vc acha?
\fvp{divulgacao do conhecimento gerado}

Others have attempted to analyze KGs in order to extract information. CAVA~\cite{cashman2020cava}, for instance, allows for the exploration and analysis of KGs through visual interaction. KG4Vis~\cite{li2021kg4vis}, on the other hand, uses the advantages of the KG structure to provide visualization recommendations. ExeKG~\cite{zheng2022exekg} uses KGs to record paths of execution within data mining and machine learning pipelines. Indeed, there is an ever-increasing number of works using KGs in VA, all of which agree that KGs are suitable for knowledge analysis and extraction. Our novelty among such works is using KGs to model the user's knowledge discovery process as paths within the KG, which are then extracted as slide decks.

\fvp{entao acho que poderiamos chamar de divulgacao da informacao em formato de slide decks. Ou algo assim.}

% ADD: lipford2010helping
Only some works have attempted to model user behavior or their knowledge discovery in a way to generate or extract slide decks. StoryFacets~\cite{park2022storyfacets} is unique in this aspect. They have developed a single system showing visualizations in dashboard and slide-deck formats. Although slide decks have well-researched limitations~\cite{knaflic2015storytelling}, they also argue about how and why slide decks are advantageous when one wishes to narrate a sequence of events. Indeed, slide decks are yet to be dethroned as the utmost way to give presentations~\cite{schoeneborn2013pervasive}. Of course, other works have succeeded in recalling and retelling the knowledge discovery process in other means~\cite{xu2015analytic}. For instance, Ragan Et.Al.~\cite{ragan2015characterizing} lists many tools that collect and structure user behavior and insights in a queriable format. Nevertheless, they all have not proposed a means to extract slide decks from their collected data to narrate the knowledge discovery process to third parties.

\fvp{ficou legal esse final. Acho que anteriormente, podemos criticar nao com base em slide decks mas - recalling and retelling the knowledge. }
TODOLC: nao eh CSCW e eh bom deixar claro, mas deixar uma pessao apresentar o que o outro fez (colocar um pouco na intro tb) (given thereis a team expoloring and aggregating insights, how to unify theyr insights to show/present to a third party like danny does?)



% add andrienko2018viewing?
%VAKG proposes to structure the knowledge gathering process within the Visual Analytics (VA) life-cycle into a set of linked knowledge graphs, constituting a \textit{Visual Analytic Knowledge Graph (VAKG)}. 

% tem q colocar https://ieeexplore.ieee.org/abstract/document/7192662 e https://ieeexplore.ieee.org/document/7042482 e https://ieeexplore.ieee.org/abstract/document/8788592?casa_token=cum9dJ9jjrMAAAAA:IKCkX3CTsuSZZyRRClLJm1sLjFTlApR73jAxd-NHqz3SNMVvK6rCKgbkYEwhttxRUtwy5txN USAR COMO BASE
% comparar com processos existentes de guardar e processar knowledge gathering (insight provenance)

% TODO: copiar RW do https://journals.sagepub.com/doi/full/10.1177/14738716211032653#fig4-14738716211032653
% add https://arxiv.org/pdf/2210.03305.pdf too: How Do Data Science Workers Communicate Intermediate Results?

% Many works have shown not just how to collect user data for analysis, but how to utilize it for the advantage of the user. 

%%%%%%%%%%%%%%%


% \textbf{Knowledge and Feedback. } The literature in knowledge modeling methodology defines the existence of a flow of insight and knowledge generation caused by the user's interactivity with the computer (Fig.~\ref{fig:teaser}(A)). Since the origin of VA, significant work has been done to demonstrate the breadth and depth of \textit{knowledge} within VA~\cite{sacha2014knowledge}. \citet{federico2017role}, for instance, describe in great detail many of such works and also define ways to interpret VA research in light of the knowledge model. These works may differ when describing VA's sub-components, such as data mining or visualization, but common to them is VA's purpose of creating insight or knowledge at the end of some workflow~\cite{federico2017role, chen2019ontological}, which is done through interactivity between the user and computer. Our work does not try to redefine any of these concepts but borrows the ones used by most~\cite{federico2017role, chen2019ontological, polowinski2013viso}, translated, in general words, as pieces of concrete information inferred by experience or learned from an external source. On the other hand, these theoretical works~\cite{sacha2014knowledge, federico2017role, polowinski2013viso} do not discuss how such models can be used to record and analyze the user's \textit{knowledge gathering} process itself.

% %\textit{Knowledge Gathering} is the terminology we adopt for tracking the user's knowledge gain as a temporal sequence of insights or findings.
% % 
% VA's knowledge model research has tackled the problem of \textit{Knowledge Gathering}, that is, tracking the user's knowledge gain as a temporal sequence of insights or findings, in many different ways. However, knowledge gathering within these works and systems is seen only as a conceptual model. \citet{federico2017role} lists many systems where a notable example is a work by \citet{keim2010mastering} which creates an application-specific knowledge gathering process by utilizing automated analysis with human interaction. Furthermore, \citet{federico2017role} also argues that since this knowledge-gathering loop is conceptual, it is ``often inconsistently used'', which shows a limitation of when this conceptual model is applied in practice.

% \citet{federico2017role} describe, however, a very well built taxonomy where we can see how the subsequent interactions and \textit{feedbacks} between the user and the computer are related. For instance, they describe how automatic processes in data mining can generate new visualizations or how machine learning can help the user understand the data itself. Such examples are also expanded into their ontological design, such as how data provenance~\cite{da2009towards}, data mining~\cite{sacha2018vis4ml}, ML explainability~\cite{spinner2019explainer}, and the visualization, which shows how their results relate to each other. However, none of these works compares the temporal aspect of knowledge gathering with the workflow's \textit{space state}. With VAKG, we attempt to fill this gap by designing an ontology that defines temporal sequences of knowledge gathering per user and explicitly links these sequences with an \textit{atemporal state space} of the feedbacks users may receive from a VA workflow.

% \textbf{Interactivity Provenance. } To better understand the concept and applicability of knowledge gathering, significant research has been done regarding \textit{knowledge provenance}, which is an approach to model the knowledge gathering process as a graph network. For instance, many works within \textit{Semantic Web} discuss ways to understand or structure knowledge provenance within the Web~\cite{da2003knowledge}. 

% Knowledge provenance is extracted from \textit{Data Provenance}, describing the sequence of changes datasets may have had over time. With provenance, the tracking of knowledge can be modeled as a change in datasets~\cite{da2009towards}, updates in visualizations~\cite{battle2019characterizing, xu2020survey} and extracted through graph network analysis~\cite{fujiwara2018concise}. Among such works, \citet{chang2009defining} attempt to use visual analysis within a Knowledge Base system, storing knowledge extracted from experts into a ``compressed'' format using a Knowledge Database. These works show examples of applying provenance to understand the knowledge gathering process. Still, although they describe ways to link knowledge gathering to user interactions, it is rare to see a differentiation between the historical sequences of user-generated events and the atemporal state space of the VA workflow. In other words, two concepts are normally merged in these works: the \textit{temporal} aspect, which indicates what and when users executed VA tasks, and the \textit{atemporal} aspect, which indicates what are the possible VA workflow states and how they transition between each other.

% \textbf{Beyond Models: Tracking and Analysis. } User-tracking and behavior analysis research has also been active. The user-tracking taxonomy of \citet{von2014interaction} models user behavior as a graph for analytical purposes. However, since these tools do not integrate directly with a knowledge model but only focus on solving a specific domain problem, the integration between tools and the existing knowledge models is rarely addressed. This causes issues when discussing the usage of these models as an ontology to store user-tracking data in a knowledge graph~\cite{fensel2020introduction}, explore it~\cite{cashman2020cava} and perform analysis over it. For instance, the interactivity taxonomy of \citet{von2014interaction} cannot be used within the descriptive ontology of \citet{sacha2018vis4ml}. They also do not discuss how multi-user VA workflows connect to \citet{battle2019characterizing}, nor allow for comparisons between the user's exploratory space when compared to their motifs~\cite{xu2020survey}. VAKG solves this by a multi-layer architecture, allowing for differing taxonomies and ontologies to live and be analyzed as separate sub-components of the graph network.

% On the other hand, existing VA systems use these taxonomies as a theoretical or conceptual background while using the user-tracking data only for specific domain use-cases. For instance, user's \textit{Tacit Knowledge}, as defined by \citet{federico2017role}, is tracked in VA by many different feedback methods, such as manual feedback systems~\cite{bernard2017comparing, mathisen2019insideinsights}, manual annotations over visualizations~\cite{soares2019vista}, and inference methods that attempt to discover the user's insights by analyzing their interactivity patterns~\cite{battle2019characterizing}. Nevertheless, they do not provide the user-tracking data as a solution to the bigger knowledge provenance problem, only to their specific domain's goals. Among these VA systems, InsideInsights~\cite{bernard2017comparing} is the only one that gets close to addressing this limitation due to its unique and well-built approach to recording insights through annotations during the user's analytical process. However, the proposed solution is not able to track automatically-generated insights~\cite{spinner2019explainer} nor account for automatic computer processes~\cite{federico2017role}. VAKG includes all these aspects in its ontology.

% Additionally, though VA systems typically attempt to apply visualization and data mining processes to solve specific problems within a given domain, the research over domain knowledge and technical knowledge concepts usually only produces conceptual models~\cite{chen2017pathways}. Such conceptual research is instrumental for the field. However, the knowledge needed to build a VA system or tool (e.g., domain and technical knowledge) and the user knowledge model of \citet{sacha2014knowledge} are ontologically disconnected~\cite{chen2017pathways}. On the other side, research of ontologies that model VA in a graph form~\cite{chen2019ontological, sacha2018vis4ml, tennekes2021design, von2019informed, chen2019ontological} does not solve the knowledge provenance problem. Therefore, although the current knowledge model framework described by \citet{sacha2014knowledge} and \citet{federico2017role} are instrumental to understanding how current VA systems produce knowledge, it by itself is insufficient to provide insights into the ongoing aggregation of knowledge throughout a VA task and, consequently, is unable to be used as the means to store the tool's usage and user's behavior and knowledge gain. VAKG attempts to bridge this by providing a flexible architecture where other's theoretical work can be incorporated into our ontology, and by exposing it as a knowledge graph, VA systems may be able to analyze their own knowledge gathering process.

% \textbf{Knowledge Graphs. } Ontological design of knowledge has been a central goal of the areas of Knowledge Bases and \textit{Knowledge Graphs} (KGs)~\cite{fensel2020introduction}. KG~\cite{chen2020review} is a widely used technique to store knowledge in a structured format and has shown many successful methods of how to interpret, store and query explicit knowledge, such as the information within Wikipedia~\cite{auer2007dbpedia}. KGs expand knowledge models' ontology by defining a specific way of structuring knowledge as relationships through a graph-based framework, which allows the ontologies discussed so far to use KGs as a means to store information within a graph database, such as neo4j~\cite{noauthororeditorneo4j}. Compared to typical databases, the structure of KGs focuses less on the usual transactional or row-based structure~\cite{cashman2020cava}. It focuses more on the types of knowledge properties and relationships between these properties. The KG ontology usually uses the OWL format~\cite{chen2019ontological, sacha2018vis4ml, von2019informed}. However, one difference is in its focus to describe the \textit{Classes} and \textit{Relationships} in light of the expected use-case of the database.

% KGs have many other parallels and connections to the overall graph research, including Graph Neural Networks (GNNs)~\cite{jin2020gnnvis}, graph visualizations~\cite{chang2016appgrouper, he2019aloha} and graph operations~\cite{ilievski2020kgtk}, such as page rank and traveling salesman. For our use-case, a notable sub-type of KGs is the \textit{Temporal Knowledge Graph (TKG)}, whose ontology is the temporal relationship of the data such as ``order of events'' or ``time difference between events''~\cite{gottschalk2018eventkg}. This technique creates a graph-based timeline of knowledge evolution. Different from the existing works, VAKG ontology is designed to focus on the analytical use-case of sequence analysis~\cite{xu2020survey}, which can be done through TKGs and graph-theory abstractions of temporal graphs.


==> paper/backup or references/4a_application.tex <==
\section{Illustration of VAKG Usage}\label{sec:extensions}

% \fvp{Não sei se o nome applications eh apropriadao ja que o que esta abaixo sao ideias de aplicacao e nao aplicacoes em si. Acho que sao mais cenarios hipoteticos de uso.}

Our first discussion of potential applications of VAKG will focus on Exploratory Data Analysis (EDA), which aims at providing users with easy access to data through visualizations and analytical capabilities~\cite{keim2010visual}. The existing Knowledge Model framework~\cite{federico2017role} describes why such EDA tools perform well by providing a platform for users to utilize their \textit{tacit knowledge} and visualizations to harness and gather new insights over time. As was already noted, most of such tools do not record the interaction of users, and even fewer record users' new insights and knowledge. However, by using VAKG, this gap can be filled.
%%%

Currently, for EDA tools to track their usage, developers heavily utilize services such as Google Analytics~\cite{clifton2012advanced}, Datadog~\cite{datadog}, Elasticsearch~\cite{Kononenko2014MiningElasticsearch}, or custom metrics recorders from the major cloud providers. These services focus on recording logs, metrics, or transactions which occur while web-based systems are used. VAKG can be used similarly. However, VAKG utilizes a relationship-first approach due to its focus on KGs. To test out how well VAKG couples with current tools being developed, the system ExPatt~\cite{christino2021explainable}, which was already using Google Analytics to track usage metrics, was used to populate a VAKG.

ExPatt is an EDA tool developed for the analysis of heterogeneous linked data, or more specifically: concomitant analysis of GapMinder data and Wikipedia documents. Fig.~\ref{fig:expatt} exemplifies the interface of ExPatt, where users can use line charts, maps, and curated lists of recommendations to explore and analyze world demographic datasets. For our example, we will follow the ExPatt paper's proposed scenario where a user investigates USA and Russia's life expectancy indicators. Namely, the user first investigates USA's life expectancy values, then adds Russia's onto the line chart for comparison, and finally verifies if the same pattern seen so far is also present in the mortality rate indicator of both countries. VAKG was populated with this usage information and can be visualized by the representation of Fig.~\ref{fig:vakgexpatt}.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{pictures/expatt.png}
    \caption{ExPatt interface setup to explore world demographic indicators. Using a line chart (A), users can select findings (B) and analyze the indicators through a world map (C). 
%ExPatt links said dataset to a separate Wikipedia database, showing its result as document overview visualizations (D, E, F, G). Also, recommendations of countries and indicators of interest related to the selected finding are given (H). 
See ExPatt~\cite{christino2021explainable} for more in-depth information.}
    \label{fig:expatt}
    \vspace{-0.5cm}
\end{figure}

\begin{figure}%[tb]
    \centering
    \includegraphics[width=\columnwidth]{pictures/VAKG abstract.png}
    \caption{A VA tool called ExPatt used VAKG to track its interface states and user's knowledge gain. The tool's state is stored as a property map, and on each update operation (e.g., an interaction on the tool) a new update node records all pertained information. Similarly the user's ongoing insights and tacit knowledge follows in a separate timeline.}
    \label{fig:vakgexpatt}
    \vspace{-0.65cm}
\end{figure}

In this example, we see in Fig.~\ref{fig:vakgexpatt} the identical $4$ sequences described in Sec.~\ref{sec:formal}, where at first the user does not have any insight and the VA tool has some visualizations, however as the user's interest is on comparing Russia and USA, the update sequence $U^{va}_t$ shows what is the interaction performed by the user, while the states sequence $C^{va}_t$ only describes what is being displayed by the VA tool at each point in time. Similarly, the two knowledge sequences on the bottom of Fig.~\ref{fig:vakgexpatt} show the user's knowledge gain as the state sequence $C^u_t$ while user interests that cause interactions with the VA tool are shown as the update sequence $U^u_t$.

In addition to the example seen so far, we also investigated the user evaluation process of ExPatt, where multiple users performed certain interactions with a specified goal. The full description of this evaluation can be seen in ExPatt's publication~\cite{christino2021explainable}. By analyzing the patterns used by users, we confirmed several of the examples of Fig.~\ref{fig:vakgexamples}. Namely, the pattern (A) was always observed when allowing for the VA tool to be used by multiple users because they always took slightly different interaction sequences with the tool, patterns (C) and (D) were observed multiple times while the users attempted to answer the survey's questions, and pattern (B) also always happened since the users took different paths while reaching the same goal with the same final answer to the survey. Furthermore, the summarization extension of Sec.~\ref{sec:summarization} was used since for the entire sequence of actions, each participant only reached one new insight in order to answer the survey. Unfortunately, if participants gained more insights during this process, ExPatt did not collect the information.

Once the graph data structure is created, graph analysis techniques can be used on top of VAKG to identify patterns in the user's analysis, suggest next-step recommendations, or suggest knowledge generated from previous users who took the same analysis paths as the current user. For instance, many users in ExPatt did not reach the survey's answer using the minimum path, but now this can be verified by using the graph theory method of minimum path analysis. This process is exemplified in Fig.~\ref{fig:vakgshortestpath}


\begin{figure}%[tb]
    \centering
    \includegraphics[width=0.8\columnwidth]{pictures/vakgshortestpath.png}
    \caption{VAKG provides graph analysis capabilities. One example is shortest path analysis, where if two users attempt to reach the same goal through different interactivity paths, VAKG will display the minimum interactivity path (left). Similarly, if two users progressively gain new insights to reach a common new knowledge, VAKG will display the minimum path of knowledge gain (right).}
    \label{fig:vakgshortestpath}
    \vspace{-0.65cm}
\end{figure}
%%%%

==> paper/backup or references/5a_examples.tex <==
\section{Hypothetical VAKG Usage}\label{sec:future}

Just as ExPatt, VAKG is a good fit for VA systems where the user has access to a dashboard of linked visualizations to perform simple data analysis, such as GapMinder~\cite{rosling2012gapminderorg}, Covid-19~\cite{bccovid}, national census websites~\cite{canadadashboard} or other similar websites such as the Datatool project~\cite{engagenovascotia}. If VAKG is set up within one of these systems, the resulting graph will contain the complete state of the dashboard at a given time $C^{va}_t$, including information of what is the data and filters selected. When the user interacts with the visual representations, the system sends the interaction information as a dictionary structure to VAKG, which generates a new update node $U^{va}_t$ following $C^{va}_{t+1} = U_t^{va}(C^{va}_t)$, creating once again many of the patterns seen in Fig.~\ref{fig:vakgexamples}. In this simple setup, the system will successfully record all interactions over time within VAKG. However, the user has no intuitive way to convey whether they have acquired any new knowledge $U^u_t$. In order to know when users identify any new insights or knowledge within their analysis, manual feedbacks (e.g., annotations) are required from the user at any/every interaction. However, in this example, we are expecting the user to provide all their tacit knowledge manually. However, if users perform multiple interactions before any new tacit knowledge feedback, the system will be required to use the \textit{update summary extension} of Sec.~\ref{sec:summarization}.

Another similar example is the usage of VAKG within statistical analysis tools~\cite{abbasnasab2021comparing}, where datasets are loaded, processed and through statistical analysis, the user can extract whether a particular hypothesis is valid or not. In order to fit this scenario to VAKG, the tool can use a similar setup where the tool state nodes $C^{va}_t$ and update nodes $U^{va}_t$ are the actions taken by the user, such as ``inclusion of dataset X'', and also use any of the statistical analysis methods applied generates new knowledge as new user nodes $C^{u}_t$ and $U^{u}_t$. This way, we expect that this VAKG would be able to explain how different users utilize a certain statistical analysis tool (Fig.~\ref{fig:vakgexamples}), whether the users are taking the optimal paths to reach the conclusions needed (Fig.~\ref{fig:vakgshortestpath}) and, of course, VAKG would also record all new knowledge generated by the users for further usage.

% \fvp{Ainda fico relutante de falar o paragrafo abaixo. Fico imaginando se formos escrever um artigo sobre exatamente isso no futuro. Pode soar estranho se os revisores souberem desse paper... eu consideraria comentar esse paragrafo...}

% There are other examples outside the realm of EDA and even VA. For instance, we are also experimenting with VAKG to store and analyze the concept of \textit{strategy} within eSports. More specifically, by utilizing the VAKG framework over the strategy and decision-making process within an event-based timeline of a famous real-time strategy eSport game called \textit{Age of Empires 2: Definitive Edition (AoE2 DE)}, we have seen that VAKG can structure one of such matches between famous players. Due to the player's tacit knowledge, the actions $U_t$ within the game are executed by following specific known strategies $C^{u}_t$ when the players consider the current state of the game $C^{va}_t$. This structure can be used to analyze this and many other temporal event sequences that occur due to the user's knowledge gathering and their actions throughout this process.

So far, we have exemplified VAKG only containing the KG itself. However, VAKG can also be interfaced with external data to track updates of specific external resources, but due to limited space in this paper, such extensions and examples were omitted. Nevertheless, in summary, in addition to tracking the states and updates of the tool $va$ and user's tacit knowledge $u$, VAKG can track updates in the dataset $D$ when it changes over time by using the update node's property map $U^{va}_t$ also to record the whole dataset state and any descriptors, such as averages and outliers, and filters within the visualizations. Another approach is to track an external dataset using hyperlinks, and in case multiple datasets $D_n$ are being used within a single VA tool $va$, VAKG can track hyperlinks to all datasets, including what partition of each dataset is being shown by the VA tool.

In the given examples, the underlying dataset does not change during analysis. However, if the dataset is the running stock market information, both the stock market price over time and the numeric differences between each of the prices over time can also be part of VAKG's state nodes $C^{va}_t$ and update nodes $U^{va}_t$, respectively. Further applications, such as weather data or user-tracking data, can be considered VA tool updates $U^{va}_t$, and information of the user's emotion from sensor data, such as 3D scanners or biometric sensors, can be considered user updates $U^u_t$. VAGK can even be applied to software analysis if the developer uses git commits, issue trackers, and user feedback to update a VA tool's code over time. 

Though we envision many examples, all follow the same process. First, we model the user interactivity and user knowledge gain from each example and then fit this model into the VAKG structure of a VA tool and user knowledge of Fig.~\ref{fig:teaser}. Although there are challenges within each example of how to best perform this fit, once it is done, we have shown that VAKG provides valuable capabilities of recording the user interaction information over time, recording the user's knowledge gain process, and analyzing usage patterns.

\vspace{-0.25cm}
\subsection{VAKGI}

As a final contribution, we also created a sample implementation of the proposed VAKG, which we call VAKGI. Though useful for testing, it is important to note that VAKGI is not the same as VAKG, but only implementation of some aspects of VAKG within a specified domain. VAKGI uses a multi-tenant web-accessible REST API architecture, allowing any tool and website to attach to and try out VAKG easily. The Python implementation of the VAKGI server~\cite{leonardo_christino_2021_5750019} connects to a Neo4J~\cite{noauthororeditorneo4j} server as the graph database back-end. The expected architecture can be seen in Fig.~\ref{fig:arch}. Using this, we have connected some existing tools created within our group for tests and analysis, such as ExPatt~\cite{christino2021explainable} and Datatool~\cite{engagenovascotia}.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{pictures/VAKG arch.png}
    \caption{VAKGI: A sample implementation architecture of the VAKG framework. With VAKGI, any VA tool can inform its $va$ updates and user's $u$ updates and states as web API calls, similar to how one would do to Google Analytics. Once some usage data is populated, the VA tool using VAKGI also has access to the graph structure through API calls and the ability to fetch information, analysis results, or visualizations directly from Neo4j.}
    \label{fig:arch}
    \vspace{-0.65cm}
\end{figure}






% \subsection{E-Sports Analytics}
% % time-data, e.g. games
% Although web-based tools seem a straight-forward example of applying VAKG, we have also utilized VAKG to store and analyse the concept of \textit{strategy}. By investigating the strategy and decision-making process within an event-based timeline of the famous real-time strategy eSport game called \textit{Age of Empires 2: Definitive Edition (AoE2 DE)}. The current state of the \textit{Definitive Edition} version of AoE2 has had many high-profile tournaments, where competitors play the game for tens of thousands of spectators through streaming platforms, such as Twitch and YouTube, for prices as high as US\$100,000.00. Matches within this game involve both prepared strategies and per-game adaptations strategies to counter the opponent. In a succinct manner, the game involves two parties building a self-sufficient economy by building entities capable of resource collection and properly managing their tasks in order to optimally collect the required resources to execute a specific strategy. In parallel, the game expects the players to use their economy to build military units and/or buildings in order to either defend their territory and resources or to attack their opponent, through which the game's winner is decided. Therefore, the game expects serious multitasking with multiple economical and military tasks being executed in parallel while the player optimally applies a prepared strategy or counters the opponent's strategy.

% We have analysed one of such matches between famous players, and by unpacking the recorded game we can extract all the executed actions from each player $U^{va}_t$. These actions are executed by following certain known strategies, which comes from the player's tacit knowledge $C^{u}_t$, or as a reaction to counter the opponent $U^u_t$. New knowledge constantly arrives to each player, which is then used to decide the next step. Therefore, we can apply the VAKG framework to each player, and by using the publicly available video-recording of one of the players, we have enhanced the VAKG graph with his own inputs of strategies and decision-making explained during the video. By using the same REST API described above, we have collected these information within VAKG and the result can be seen in Fig.\ref{fig:TODO}, from which we can see the entire game at a glance. Similarly to the EDA systems, once VAKG stores the structure, all graph analysis techniques can be used to provide recommendations, suggestions and insights over strategies and decision making. Further research is planned in order to fully analyse how VAKG can help players and spectators to understand the strategies used and to hone their skills. For this, we plan to invest into developing a visualization which explains the relationship data of VAKG so that domain-specific users can utilize VAKG as an analysis platform as well.

% % VIZ
% We recognize that the visualizations of VAKG presented so far has demonstrated a severe limitation of this framework. Although there are many methods of visualizing simplified graphs such as trees, acyclic graphs and flow charts, the complex nature of visualizing the entire VAKG knowledge graph, or even a specific partition of a single user's information, for example, was found to be a difficult task. This process is planned as one of our major next steps in order to allow for visual analysis capabilities of VAKG in addition to the already present algorithmic-based analysis, such as page-rank and recommendations.

% simple analysis example(s)
%% EDA

==> paper/backup or references/5b_interviews.tex <==
\section{VAKG in Practice:  Domain Expert Interviews}\label{sec:interview}

During the development of VAKG, Janio was kind enough to give inputs related to the usefulness of tracking user interactivity for knowledge gain. Janio is an experienced entrepreneur and business owner in the international food supply chain as an international food importer and wholesaler, and regional restaurant chain ownership and management with over 30 years of experience. The hour-long interview focused on his methods to store information and extract knowledge from Enterprise Resource Planning (ERP) and Accounting systems. In summary, he said the usual process depends heavily on training employees to record sales manually and restocking data in a system. Once the data is stored and structured into a timeline of events, he generates reports and uses his own business experience to discover and explain insights from the data. We have included a small excerpt of the interview below.

\textit{Q: Can you give examples of when and how you use provenance and analysis?} 
%
One example is how I analyze the product purchase behavior of select customers on a month-to-month basis and the overall monthly product-based sales compared to previous years. I do this by extracting all reports from my accounting software and using MS Excel to merge them and analyze the result, sometimes on a month-by-month basis or a year-over-year basis, depending on what I am analyzing. (...) Among the main difficulties within the process is the required expectation of correct imputation by the employees and the amount of external knowledge I need to bring to the report so that analysis can be meaningful. In our restaurants, employees would input the payment type of a purchase, such as cash or credit card. However, once the customer makes the payment, sometimes the type would swap, but the system is not updated, causing many discrepancies in the monthly accounting process.

\textit{Q: How external knowledge was used and was it included in the reports?} 
%
(...) managers typed in manually certain events, such as heavy rain or large soccer match, while inputting the weekly restocking information. (...) however, most of the time, the external knowledge I use is either only manually typed during the analysis itself after the generated report or not included at all, just coming from my head, experience, and the internet.

%\subsection{Data Scientist Interview.} 
We also interviewed Thiago, a Data Science General Manager of Credit Recovery in a large bank. Thiago has a Ph.D. in Machine Learning applied to Natural Language Processing and has over a decade of industry experience in applied data science. In summary, we discussed in his interview the past and present use of provenance analysis within decision-making processes.

\textit{Q: Can you give examples of when and how you use provenance and analysis?} 
%
Bank transaction provenance, such as payments and money transfers, is extensively used for flagging fraudulent transactions. (...) My area then uses machine learning to predict the tendency of credit repayment. The treatment of temporal relationships of the data, such as order of transactions, is sometimes part of an embedding step or forwarded to a machine learning model which can handle temporal data. A new project in my area uses provenance to better design a data science workflow. Currently, our bank does not have a well-optimized data analysis workflow. Still, by tracking the data analysis, we plan to record the work effort of each task and, in the future, analyze the results to improve the overall workflow or help us plan the future by predicting how long data analysis tasks will take.

\textit{Q: Would a temporal knowledge graph structure, such as the one from VAKG, aid in such applications? How? } 
%
A co-worker and I have been investigating using a knowledge graph representation of customers that could describe behavioral patterns for better predictions during fraud analysis. (...) Another large intersection I see is by using such a structure to record and analyze our Data Science pipeline. Using such recording, we envision predicting a more optimized sequence of tasks required for a new data science project given a description of goals or problems we want to solve.

We use these interviews to check in the wild the significance of our motivation, goals and get insights into future works for VAKG when applied to real business analytical processes. For instance, Janio confirmed that his experience with ERP and accounting software essentially had data provenance but rarely tracked any external information at the time when the data was changed, such as the reasoning of why his employee changed the data (\textbf{G1}). Janio said he manually had to track down these extra pieces of information through an involved and time-consuming cross-check process and use external software to merge and analyze it (\textbf{G2} \& \textbf{G3}).

Similarly, Thiago's usage of provenance requires significant work by data scientists for analysis to process the data (\textbf{G2} \& \textbf{G3}), and his wish to better understand this data science pipeline through provenance and knowledge graphs indicates both the lack and the potential of using VAKG (\textbf{G1}). These examples show that VAKG's focus on tracking the user's knowledge gain in tandem with user interactivity aims to aid in this problem: the analysis of data-oriented workflows that requires or would benefit from the connection between data provenance, external data (e.g., supply chain or bank transactions) and user knowledge gain (e.g., intentions and behavior).

==> paper/backup or references/sketch.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018


\title[Knowledge Graphs and Dataspaces in Visual Analytics, a Survey]%
      {Knowledge Graphs and Dataspaces in Visual Analytics, a Survey}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[L. Christino \& F. Paulovich]
{\parbox{\textwidth}{\centering L. Christino$^{1}$\orcid{0000-0002-8754-8460}
        and F. Paulovich$^{2}$\orcid{0000-0002-2316-760X} 
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$Dalhousie University, Canada\\
         $^2$Eindhoven University of Technology (TU/e), Netherlands
       } 
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

% \teaser{
%  \includegraphics[width=\linewidth]{eg_new}
%  \centering
%   \caption{New EG Logo}
% \label{fig:teaser}
% }

\maketitle
%-------------------------------------------------------------------------
% \begin{abstract}
%   User-guided knowledge generation is considered one of the core concepts of Visual Analytics (VA), but this concept is considered abstract within VA application development. At the same time, the act of structuring and analyzing knowledge as knowledge graphs or through dataspaces has shown that data and its derived insights can be structured for analytical purposes. In order to broaden VA research, this survey will discuss existing publications within the three areas of research from the viewpoint of user-guided knowledge generation. For this, we provide a structured, systematic, and accessible mapping of usages of knowledge graphs and dataspaces within the context of VA by analyzing and categorizing relevant literature. Finally, we will end by discussing ways where existing research can be used across the other fields and current challenges and research gaps.
% %-------------------------------------------------------------------------
% %  ACM CCS 1998
% %  (see https://www.acm.org/publications/computing-classification-system/1998)
% % \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% % \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% % \end{classification}
% %-------------------------------------------------------------------------
% %  ACM CCS 2012
% %   (see https://www.acm.org/publications/class-2012)
% %The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% % CCS codes.
% %Example:
% \begin{CCSXML}
% <ccs2012>
%   <concept>
%       <concept_id>10003120.10003145.10003147.10010365</concept_id>
%       <concept_desc>Human-centered computing~Visual analytics</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
%   <concept>
%       <concept_id>10010147.10010178.10010187</concept_id>
%       <concept_desc>Computing methodologies~Knowledge representation and reasoning</concept_desc>
%       <concept_significance>300</concept_significance>
%       </concept>
%   <concept>
%       <concept_id>10010147.10010178.10010187.10010193</concept_id>
%       <concept_desc>Computing methodologies~Temporal reasoning</concept_desc>
%       <concept_significance100</concept_significance>
%       </concept>
%   <concept>
%       <concept_id>10010147.10010178.10010187.10010195</concept_id>
%       <concept_desc>Computing methodologies~Ontology engineering</concept_desc>
%       <concept_significance>100</concept_significance>
%       </concept>
%  </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Human-centered computing~Visual analytics}
% \ccsdesc[300]{Computing methodologies~Knowledge representation and reasoning}
% \ccsdesc[100]{Computing methodologies~Temporal reasoning}
% \ccsdesc[100]{Computing methodologies~Ontology engineering}


% \printccsdesc   
% \end{abstract}

\maketitle
\section{Introduction}
% \firstsection{Introduction}
% \maketitle

One of the main components of any Visual Analytics (VA) tool is to allow user-guided data analysis. This process is known to be guided by user interactivity towards knowledge generation~\cite{sacha2014knowledge}. The understanding of what knowledge is, how it is formed, and how one can model such knowledge generation into a shareable format has been much investigated within Visual Analytics (VA)~\cite{collins2018guidance} and Knowledge Graphs (KGs)~\cite{chen2020review} fields. For instance, \cite{collins2018guidance} describe in detail what intelligent guidance is and how it provides digestible and interpretable information to users from visualizations. 
For instance, a tool applies intelligent guidance by reducing the cognitive load and visual bias that users interacting with a visual analytic tool may experience. 
Since the analysis of users' behavior is dependent on their pre-conceived tacit knowledge~\cite{federico2017role} and their own interest when starting an analysis process, \cite{collins2018guidance} also describe a knowledge model where VA is the means for users to generate and amass knowledge through visual interactivity. In this context, the authors describe KGs as a representation of user-generated knowledge. 

Explicit knowledge, however, is treated differently. Since this type of knowledge is defined as what is explicitly described within a dataset~\cite{federico2017role}, visualizations employ visual artifacts, such as annotations or bookmarks, to encode an \textit{explicit representation of knowledge} as part of a tool~\cite{federico2017role} or encoded as a data-structure, such as a Knowledge Graph (KG). In order for a KG to provide value for users, the literature classifies the usage of KGs into three distinct reasoning types~\cite{chen2020review}: rule-based reasoning, distributed representation-based reasoning, or neural network-based reasoning. Although KGs are used within applications such as recommender systems, health analysis systems, fintech, and question-answering systems~\cite{chen2020review}, each individual application use KGs in different ways. In short, we see KGs being interpreted as both an abstract representation of user-generated knowledge~\cite{collins2018guidance} and a graph-structured data model to store interlinked concepts~\cite{chen2020review}. 

While KGs provide a single source where to store and structure knowledge, VA thrives in situations where users are required to use interactivity for gradual aggregation of insights, findings, and knowledge~\cite{sacha2014knowledge, federico2017role}. As part of the gradual process of VA, data analysts are required to source multiple datasets and perform well-known data mining steps, such as pre-processing and cross-analysis, before the creation of a visualization solution. The area of DataSpaces (DSs), however, focuses on the understanding and analysis of multiple heterogeneous datasets an integral part of the analytic process~\cite{collins2018guidance, golshan2017data} instead of delegating to only a pre-processing step. 
Indeed, DSs have been emerging as one of the cornerstones of data integration and storage tasks~\cite{golshan2017data}, especially when applied to multiple heterogeneous datasets, such as text, tabular, and video datasets. 
In short, a DS~\cite{franklin2008first, franklin2005databases} is a concept that aggregates any number of datasets into a single unified service in a pay-as-you-go fashion. At its core, a DS provides a platform where you can store and query any number of datasets, and, as you gather more information from the said datasets, you progressively add links between datasets 
, features of the data, additional extrapolated features,
or any new information \textit{as-you-go}. These links can themselves be stored in a graph structure~\cite{chen2020review}. DSs have shown to be advantageous when processing and analyzing a combination of stream data, IoT data, heterogeneous data or large datasets~\cite{franklin2005databases, singh2011survey, curry2020real}.

In this context, KGs have been shown to pair well with DSs~\cite{beheshti2018corekg} in order to allow a multi-level loose data linkage pattern. Also, the DS's \textit{pay-as-you-go} mindset can be considered similar to VA's gradual aggregation of knowledge through user interactivity. 
However, a combined solution has yet to be seen within visualization or exploratory data analysis contexts, which are core components of VA.
Therefore, in this state-of-the-art report, we provide a structured, systematic, and accessible mapping of usages of KGs and DSs within the context of structuring and analyzing knowledge among the VA literature by analysing the most relevant research found in VA which involves the usage of the discussed concepts. 
Some of the questions we answer are: 
\squishlist
    \item What strategies have been employed to utilize KG and DS techniques to develop VA tools?
    \item How does one visualize KG and/or DS concepts/data within an exploratory visual data analysis context and with what goals?
    \item How does the user's gradual accumulation of knowledge within VA compare to KG and DS and how do they differ?
    \item What are the state-of-the-art methods to structure and analyze explicit and tacit knowledge?
    \item Which challenges are still not solved?
\squishend
We believe our survey will prove useful to researchers of all three fields: VA, KG and DS, as an overview of the intersection of the fields and as a reference list of challenges and gaps in the literature. 

% We believe our survey will prove useful to a varied audience, such as KG and DS researchers who need an overview of how the area pairs to current open challenges within VA; VA researchers when developing or benchmarking new visual and interactive solutions which either use a knowledge framework as a core component during development or make use of multiple heterogeneous datasets; and domain-specific researchers who use (or would like to use) visualizations of KG algorithms with heterogeneous data as a method for effectively performing data analysis.

\section{Related Surveys}

The application of DSs is discussed by several surveys~\cite{kasamani2013survey, curry2020real} and can be partitioned between a catalog and browser of datasets, a unified queryable repository of datasets, and a stream funnel of real-time datasets. For example, \cite{curry2020real} discusses DSs for real-time Internet of Things (IoT)-based sensors. Further usages of DSs are personal information management, personal health management, Science, and, arguably, the web itself~\cite{franklin2008first}. The concept of linking data is also found in Data Integration (DI), a separate vast research field which includes surveys in the context of VA such as entity matching~\cite{kopcke2010frameworks}, entity resolution~\cite{kang2008interactive}, entity deduplication~\cite{morton2016view, muelder2016visual, kang2008interactive, bilgic2006d} and semantic resolution~\cite{savelyev2014interactive, li2021kg4vis, moreauvisual}. Although we see some surveys and research articles that discuss KGs and DSs, we have yet to bridge the gap of how visualizations and VA can benefit from these areas. Therefore, it is advantageous for us to analyze the intersections of these areas with VA and expose the benefits they may bring.

Among the many applications of KGs, we find surveys originating from Semantic Web~\cite{ferrara2011data} that discuss loosely linking many heterogeneous datasets~\cite{zou2020survey, nguyen2020knowledge, auer2007dbpedia}. Of course, KGs have many other parallels and connections to the overall graph research, including Graph Neural Networks (GNNs)~\cite{jin2020gnnvis}, graph visualizations~\cite{chang2016appgrouper, he2019aloha} and graph network operations~\cite{viegas2004social}. However, the concept of using KG to store and analyze the user's knowledge-gathering process is still somewhat unknown within VA, and although many publications tackle the broader \textit{Knowledge Generation} problem~\cite{wang2016survey, federico2017role}, and others attempt to perform a visual analysis of existing KGs~\cite{chang2009defining, xu2020survey}, there is not much effort into utilizing KG within VA itself. We intend to discuss this limitation and provide a clearer distinction and definition of KG, its core concepts, and its potential use cases within VA. 

There are many other similar concepts, such as databases, networking, multi-dataset machine learning, time-series machine learning, graph-neural-networks, and others, however, we will limit our survey to the intersection of the three areas while also exemplifying under-exploited venues of research. 

\section{Relevance to the Community}

Similar to how the term ``Visual Analytics'' may sometimes be misinterpreted or misused in other fields of study, we found that many usages of terms like ``graphs'', ``knowledge modeling'', and ``multiple heterogeneous datasets'' within VA literature have been disparate from their respective research fields. This has left much potential research utilizing said concepts unexplored. A simple search of publications of the term DSs within TVCG shows that it is only used as a ``virtual reality space'' for some VA articles and nothing more, and similarly the term ''Knowledge Graphs'' is used loosely as a ``visualization of knowledge'' instead of understanding ``graph'' as in graph networks. It is not just hard to find connections between the fields, but the number of those found shows a lack of activity which deserves more attention.

There are many possible stakeholders that may be interested in our survey, among which the most prominent are VA researchers and developers themselves. During VA development, many limitations related to DS are brought up, such as limitations on data accessibility, data quality, and data linkage. 
% Also, the concept of \textit{knowledge} within VA is almost always treated as a theoretical aspect during development, but not as a tool to be used within the development itself. 
Therefore, future developments of graph-based visualizations of knowledge~\cite{he2019aloha}, heterogeneous linked data~\cite{de2020quedi} and graph network applications in VA~\cite{wu2016survey} would be aided with our survey. By referring to our survey, these researchers would have an overview of the three areas of interest and what are the potential under-researched overlaps between the areas. Furthermore, many of these authors either are not core visualization researchers or are specialized in visualizations and, thus, our research attempts to bridge this gap through a list of applications of KGs and DSs within a VA context.

\section{Review methodology}

Relevant and recent surveys and books from the fields of KGs~\cite{chen2020review} and DSs~\cite{singh2011survey, kasamani2013survey, curry2020real} were used to identify both the overview of the area and the current state-of-the-art research. In addition, surveys in knowledge modeling, theoretical discussions of knowledge, heterogeneous dataset data-mining, and data linkage within VA journals and conferences (VIS, EuroVis, TVCG, and CGF) were also used to bring into perspective the current usage of KGs and DSs concepts within VA. We follow similar approaches presented by ~\cite{chatzimparmpas2020state}. Examples of papers selected are ~\cite{cashman2020cava, collins2018guidance, li2021kg4vis}.

The proposed structure of the survey will be a systematic one. After presenting a succinct overview of each area, we will collect the concepts which intersect KGs, DSs, and/or VA, such as \textit{heterogeneous data processing} or \textit{recording user-generated knowledge}, from a preliminary analysis of the current research being done and then will categorize the relevant literature onto the usage or not of these concepts. In addition to complexity and novelty, the structure will account for the conceptualization of knowledge~\cite{wang2016survey, federico2017role, wang2018ripplenet, ferrara2011data, golshan2017data} to link the three core areas of the survey. The results of this categorization will provide a clear map of how the current research is and what are opportunities where more attention is deserved. Further discussion of challenges and potential ideas will be given in order to inspire and prepare researchers to fill this gap. %For this, we will analyze and categorize the most relevant research found in VA which involves the usage of KG and DS concepts. Similarly, we will also categorize them by their objective type in an attempt to show any bias toward specific objectives as well as gaps of potential research objectives when considering the classification of each area described previously.
% For that, we will analyze and categorize the most relevant research found in VA which involves the usage of concepts from KGs, such as knowledge reasoning and graph-based relationship analysis, and DSs, such as the gradual accumulation of new information during the analysis of multiple heterogeneous datasets. We will also categorize the literature as by their objective type in an attempt to show any bias toward specific objectives as well as gaps in potential research objectives when considering the classification of each area. 


\section{Planned Structure}

The envisioned structure of the paper is as follows: (1) an introduction providing the usual overview, which accounts for the purpose of the paper, its motivation, and its research contributions;(2) a background with an in-depth description of the context, i.e.,
Knowledge Bases, KGs, DSs, Data Integration, and other related concepts; (3) related work for describing similar surveys and how ours differentiates from them; (4) a review methodology explaining how the literature review has been carried out; (5) a description of the categorization developed and used for the systematic review; (6) the state-of-the-art as seen through the lens of the categorization; (7) challenges and discussions; and (8) opportunities for future research.
%
% \fvp{vc olhou a estrutura dos STAR surveys existentes? A coisa mais important em um survey sao os challenges and opportunities. Essa deveria ser uma secao a parte.}
%

% \acknowledgments{}

\nocite{*}
% bibtex
\bibliographystyle{eurovisDefinitions/eg-alpha-doi}  
\bibliography{references}
%\bibliography{egbibsample}        

% biblatex with biber
% \printbibliography   

% \bibliographystyle{plainnat}
% \bibliographystyle{abbrv}
% \bibliographystyle{abbrv-doi}
%\bibliographystyle{abbrv-doi-narrow}
%\bibliographystyle{abbrv-doi-hyperref}
%\bibliographystyle{abbrv-doi-hyperref-narrow}

% \bibliography{references}


\section*{Short Biography of Authors}
\section*{Leonardo M. F. Christino}
Leonardo M. F. Christino is a PhD student in the Visual Analytics and Visualization lab at the Faculty of Computer Science, Dalhousie University. Before starting his PhD, he worked as a Back-end Engineer in several Brazilian companies finally moving to Canada to work at Amazon.com. Also with a masters in Robotics from the University of São Paulo, Brazil (2013-2016), he has researched and developed data processing pipelines and visual analytics tools in a multidisciplinary manner with the focus on data analysis democratization. For this, he has used machine learning, data processing, and visualization tools and techniques in multiple computing environments, from embedded systems to cloud computing, and adapted them to fit applications such as mobile robotics, game development, embedded systems, and interactive exploratory data analysis. In the past few years, his primary focus has been on understanding the concept of user knowledge in theory and in practice, and from these experiments, he is designing and developing visual analytics frameworks and systems to be easily accessible to the general public, all in order to encourage developers and researchers to retain and use user-generated knowledge to enhance data analysis and its applicability.

\section*{Fernando V. Paulovich}
Fernando V. Paulovich is an Associate Professor in Visual Analytics for Data Science at the Department of Mathematics and Computer Science, Eindhoven University of Technology (TU/e), the Netherlands. Before moving to the Netherlands, he was a Professor and Canada Research Chair at Dalhousie University, Canada (2017-2022), and an Associate Professor at the University of São Paulo, Brazil (2009-2017). He has been researching information visualization and visual analytics, focusing on integrating machine learning and visualization tools and techniques, taking advantage of the automation provided by machine learning approaches, and user knowledge through interactions with visual representations to help people understand and take advantage of complex and massive data collections. In the past years, his primary focus has been on designing and developing visual analytics techniques for the general public to advance the concept of data democratization, promoting unconstrained access to data analysis and widening the analytic capability of lay users in transforming data into insights.

\end{document}
